LigBench: A Unified and Human-Aligned Benchmark for LLM-based Research Idea Generation

With the rapid advancement of large language models (LLMs), research idea generation has attracted increasing attention. Existing approaches enable LLMs to retrieve relevant literature and propose novel ideas for research areas. However, current evaluation practices for idea generation remain fragmented and lack objective standards, often relying on direct LLM scoring, which limits their ability to provide unified and reliable assessments across a coherent distribution of generated ideas. To address this challenge, we propose LigBench, an automated evaluation benchmark that enables fine-grained and reliable evaluation of AI research ideas, consistently applicable across different generation distributions. In addition, we introduce PAIR-IQ, a dataset tailored for training pairwise idea judgment models and serving as an auxiliary reference to support more objective comparative evaluation. Extensive experiments demonstrate that LigBench achieves stable and interpretable evaluations, significantly improving alignment with expert judgments. Furthermore, models trained on PAIR-IQ exhibit enhanced ranking accuracy and robustness, establishing a principled standard for scalable and objective research idea assessment.

==> text/1.introduction.tex <==
\section{Introduction}

% \run{2026.1.4 Rewrite Introduction today.}

% The rapid evolution of LLMs\cite{gpt4, gemini2.5, qwen3} has ushered in a new era for automated research idea generation. By leveraging vast repositories of scientific literature, modern LLMs can propose novel hypotheses, methodological variations, and potential extensions for a wide range of scientific topics. Such capabilities hold great promise for accelerating discovery across disciplines, guiding researchers toward unexplored directions, and reducing the time and cost associated with manual ideation. However, as the utility of these systems grows, so does the need for rigorous, objective evaluation methods that can quantify the quality of generated ideas in a reproducible manner.

The rapid evolution of LLMs~\cite{gpt4, gemini2.5, qwen3} has ushered in a new era of automated research idea generation. Building on the strong reasoning and knowledge synthesis capabilities of these models, a growing body of recent work~\cite{hypothesis, aiscientist, researchagent, manyhead} has proposed LLM-based frameworks for scientific ideation, enabling the generation of novel hypotheses, methodological variations, and promising research directions grounded in large-scale scientific literature. Such capabilities hold great promise for accelerating discovery across disciplines, guiding researchers toward unexplored directions, and reducing the time and cost associated with manual ideation. However, as the utility of these systems continues to grow, the lack of rigorous, objective, and reproducible evaluation methodologies remains a critical bottleneck for the systematic assessment of generated ideas.

% In the idea generation task, an LLM is prompted with a scientific context, such as a background description, a set of research questions, or preliminary experimental results, and produces one or more candidate ideas. These ideas may take the form of new experimental protocols, alternative theoretical models, or entirely fresh research questions. Even though LLMs can match or even surpass human experts in suggesting plausible research directions under certain conditions, yet the evaluation of these outputs remains a significant bottleneck. Without standardized metrics, it is difficult to compare different models, track progress over time, or identify which aspects of generation require further improvement.

Current evaluation strategies for idea generation are often fragmented. Some studies~\cite{nova, canllm} rely on direct scoring by LLMs, where models assign quality scores to their own or peer-generated ideas, while others~\cite{scipip, nova} depend on human experts to perform pairwise or ranking-based evaluations. Automated metrics such as novelty, diversity, or semantic similarity offer partial insights but fail to capture the multi-dimensional nature of research idea quality. Overall, these approaches lack consistency: they may be sensitive to prompt phrasing, suffer from inter-annotator variability, or provide only relative assessments. Consequently, there is no unified framework to benchmark idea generation systems comprehensively.

% 这一段和上一段的逻辑关系链接不太好，感觉有点儿突兀
Pairwise comparison has emerged as a promising approach to sidestep some subjective biases inherent in absolute scoring. In this paradigm, two candidate ideas are presented side by side, and an evaluator (whether human or automated) selects the one deemed superior along specified criteria. Aggregating multiple pairwise comparisons can yield a ranking of ideas with higher consistency than solitary ratings. Nevertheless, pairwise evaluation alone does not constitute a full benchmarking solution: it requires a sufficiently large and diverse pool of test pairs, clear annotation protocols, and scalable tooling to collect judgments at scale.

To address these challenges, we introduce LigBench, an automated evaluation framework tailored for research idea assessment. LigBench operationalizes multi-dimensional quality criteria by orchestrating large-scale pairwise comparisons, metadata tracking, statistical aggregation, and automatic score updates into a cohesive pipeline. We drew on the thinking process experts use when evaluating an idea. Experts typically begin by searching for existing results related to the idea for reference or comparison. In addition, pairwise comparison alone is not sufficient to objectively and convincingly reflect the quality of an idea. Therefore, we have designed and provided a complete process based on pairwise comparison combined with the Elo mechanism to continuously update scores. We also present the PAIR-IQ dataset, a curated dataset of research idea pairs annotated across the core dimensions by domain experts. PAIR-IQ serves both as a gold-standard reference for comparative evaluation and as a training resource for models designed to predict pairwise judgments. 

Our main contributions are summarized as follows:

\begin{itemize}
    \item \textbf{Unified Evaluation Framework:} We introduce LigBench as a unified and extensible evaluation framework that systematically integrates data curation, idea retrieval, pairwise comparison, score propagation, and result aggregation within a single automated pipeline.
    \item \textbf{PAIR-IQ Dataset:} We release PAIR-IQ dataset, comprising over 15000 conference papers with debiased evaluation scores and formalized representations to support objective assessment of research ideas.
    \item \textbf{Open-Source Resources:} We will release the PAIR-IQ dataset together with the complete LigBench evaluation pipeline to facilitate reproducibility and enable community-driven extensions. The PAIR-IQ dataset is publicly available at \url{https://huggingface.co/datasets/USER3IjEBHj9/PAIR-IQ/tree/main}. The full LigBench evaluation pipeline will be released in the near future. 
    \item \textbf{Benchmarking and Analysis:} We conduct extensive experiments with state-of-the-art LLMs, demonstrating that LigBench can discern subtle differences in idea quality and offering insights into model strengths and weaknesses.
\end{itemize}

==> text/2.relatedwork.tex <==
\section{Related Work}
% \run{2026.1.4 Rewrite Related Works today.}
% The growing emphasis on AI agents and retrieval-augmented generation (RAG) to support scientific discovery and idea generation has intensified the need for robust evaluation frameworks for AI-generated ideas. The success of general-purpose large language models (LLMs) has evoked methodologies leveraging their feedback capabilities for other models. This approach, termed LLM-as-a-Judge, enables the absolute evaluation for idea assessment. Recent systems (e.g., The AI Scientist) automate multi-dimensional evaluation of generated ideas using LLM reviewers, applying diverse metrics (e.g., novelty, feasibility, impact). Crucially, human feedback is usually integrated or attached throughout these processes to ensure alignment with expert judgment and maintain evaluation reliability.

% In addition to absolute evaluation, previous studies also threw eyes on approaches such as the Idea-Arena Paradigm to acquire relative evaluation. Inspired by arena benchmarking for model outputs, the **Idea-Arena** framework ranks ideas through pairwise comparisons. Here, LLM or hybrid human-AI judges iteratively pit ideas against each other, prioritizing comparative strength over scalar scores. While sometimes absolute evaluation by LLMs tends to get  This approach inherently handles open-ended tasks lacking ground-truth answers and lack of differentiation in standalone rating systems. \cheng{Rewrite. A brief introduction without motivation. One sentence for each previous method.}

Current LLM-based ideation systems typically employ evaluation protocols that are tightly coupled to their own generation pipelines, reflecting framework-specific assumptions rather than a unified or standardized assessment methodology. Existing approaches primarily rely on either direct scoring by large language models or judgments from human experts, and are often designed to operate only within the context of a particular ideation system. As a result, these evaluation methods lack the flexibility and generality required for consistent assessment across different models, prompting strategies, and idea distributions. For instance, SciPIP~\cite{scipip} relies on evaluations conducted by human researchers, limiting scalability and reproducibility. AI Idea Bench~\cite{ideabench} introduces an evaluation protocol that is heavily dependent on the underlying idea generation framework and does not support standalone assessment of individual ideas. CoI~\cite{coi} proposes a pairwise comparison approach, but restricts evaluation to comparisons among generated ideas, making objective comparison with human-authored research ideas challenging. Consequently, as highlighted by a recent survey~\cite{survey}, evaluation remains the most critical bottleneck in LLM-based scientific ideation.

==> text/3.method.tex <==
\section{Method}
To provide a unified, objective, and human-aligned evaluation of research ideas, we propose \textbf{LigBench}, an automated benchmark designed for systematic idea assessment. As illustrated in Figure~\ref{fig:ligbench_pipeline}, the evaluation of each idea is decomposed into four aspects: \textit{rating}, \textit{contribution}, \textit{soundness}, and \textit{novelty}. Here, \textit{rating} represents the overall quality as perceived by reviewers, \textit{contribution} reflects the significance of the idea within its research domain, \textit{soundness} captures methodological rigor and validity, and \textit{novelty} measures the originality of the proposed idea.

\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth,trim=0 0 0 0,clip]{acl-style-files-master-2/figure/pipeline.pdf} \hfill
  \caption {Overview of the LigBench evaluation pipeline. Given a target idea, LigBench performs idea formalization, retrieves related papers, conducts LLM-based pairwise comparisons, and iteratively updates scores using PAIR-IQ until convergence across multiple evaluation dimensions.}
  \label{fig:ligbench_pipeline}
\end{figure*}

Following the pipeline shown in Figure~\ref{fig:ligbench_pipeline}, each idea is first transformed into a formalized representation and then iteratively compared against similar papers retrieved from the database using a large language model. In each comparison, the model evaluates the relative quality between idea pairs, and the resulting judgments are aggregated with the objective scores from the PAIR-IQ dataset to update the score of the target idea. This process is repeated until convergence, producing a final score that is consistent across different sources and aligned with human preferences.

\subsection{Idea Formalization}
To begin with, a fundamental challenge in building a unified idea evaluation framework is the heterogeneity in the formats of the ideas under evaluation. Due to inherent differences in the distributions of ideas generated by different models and frameworks, directly comparing these ideas is prone to bias. For instance, when using large language models as evaluators, they often tend to favor ideas that are described in greater detail, potentially overlooking those that are more concise yet fundamentally more innovative or valuable. Moreover, different studies are conducted under diverse frameworks, leading to substantial variations in how final ideas are presented, including their structure and formatting, which further complicates fair and consistent comparison across models and methods.

To mitigate these issues, it is necessary to standardize ideas across different distributions. Here, we focus on the core aspects and boundaries of each idea and decouple it into four distinct components:
\begin{itemize}
    \item \textbf{Main Target}: a concise, one-sentence summary of the task and objective that the idea aims to address.
    \item \textbf{Core Breakthrough}: the key advancement or novel contribution introduced by the idea compared to prior work.
    \item \textbf{Innovative Methods}: the concrete methodological approaches or techniques proposed to achieve the target.
    \item \textbf{Experimental Design}: the experimental setup and evaluation plan designed to validate the effectiveness of the proposed methods.
\end{itemize}

Formally, let $I \in \mathcal{I}$ denote an input idea from the idea space. We define an LLM-based decomposition operator $\mathcal{D}_{\text{LLM}} : \mathcal{I} \rightarrow \mathcal{T} \times \mathcal{B} \times \mathcal{M} \times \mathcal{E}$ such that
\begin{equation}
\label{eq: formalize}
(T, B, M, E) = \mathcal{D}_{\text{LLM}}(I),
\end{equation}
where $T \in \mathcal{T}$ represents the main target, $B \in \mathcal{B}$ denotes the core breakthrough, $M \in \mathcal{M}$ corresponds to the innovative methods, and $E \in \mathcal{E}$ specifies the experimental design. This formulation casts idea formalization as a structured, LLM-driven mapping into a unified representation space, facilitating systematic comparison and subsequent quantitative evaluation. The concrete prompting strategy used for this formalization is provided in Appendix~\ref{app: formalization}.

By explicitly disentangling complementary semantic facets of an idea into structured components, this LLM-driven decomposition yields a unified yet fine-grained representation that captures the substantive content while abstracting away superficial variations in expression and format. Consequently, it mitigates evaluation bias arising from heterogeneous idea sources and presentation styles, enabling more objective and consistent comparison across models and frameworks. Furthermore, this structured representation establishes a principled foundation for subsequent quantitative analyses, including assessments of soundness, novelty, contribution, and other relevant criteria.



\subsection{PAIR-IQ Construct}
% To better evaluate research ideas according to human preferences, we collected and constructed the PAIR-IQ dataset, comprising over 11,000 papers from ICLR 2024, ICLR 2025, and NeurIPS 2024, including spotlight, oral, poster, and rejected papers. For each paper, we retrieved ratings, contribution scores, and soundness scores from OpenReview. The dataset was further processed through idea formalization(as described in the previous subsection), score debiasing, and embedding computation, ensuring standardized representations and reducing subjective bias in subsequent evaluations.

To better evaluate research ideas according to human preferences, we collected and constructed the \textbf{PAIR-IQ dataset}, comprising over 15,000 papers from \textbf{ICLR 2024, ICLR 2025, and NeurIPS 2024}, including oral, spotlight, poster, and rejected papers. For each paper, we retrieved \textbf{ratings, contribution scores, and soundness scores from OpenReview}, and projected each score to a standardized 0--5 range to ensure comparability across different venues and scoring scales.

Figure~\ref{fig:dataset_statistics} illustrates the composition of the PAIR-IQ dataset. As shown in Figure~\ref{fig:conf_dist}, the dataset draws from three major machine learning venues, with NeurIPS 2024 contributing the largest proportion (49.9\%), followed by ICLR 2025 (26.6\%) and ICLR 2024 (23.5\%). Figure~\ref{fig:category_dist} presents the distribution across acceptance categories: poster papers constitute the majority (65.2\%), followed by rejected submissions (27.8\%), spotlight papers (5.2\%), and oral presentations (1.8\%). This distribution ensures that the dataset captures a wide spectrum of paper quality levels, from top-tier accepted works to borderline and rejected submissions. Figure~\ref{fig:topic_dist} further depicts the topical diversity of the dataset, spanning 12 research areas. Large language models (LLM) represent the most prevalent topic (19.3\%), followed by training methodologies (15.4\%) and reinforcement learning (13.4\%), reflecting the current research trends in the machine learning community. Detailed information and a specific example of the dataset are provided in Appendix~\ref{app:PAIR-IQ extra information}.

\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/sta3.pdf}
        \caption{Distribution by acceptance category.}
        \label{fig:conf_dist}
    \end{subfigure}
    \hfill
    % \begin{subfigure}[b]{0.48\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figure/sta1.png}
    %     \caption{Distribution by conference venue.}
    %     \label{fig:category_dist}
    % \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/sta2.png}
        \caption{Distribution by research topic.}
        \label{fig:topic_dist}
    \end{subfigure}
    \caption{Statistical overview of the PAIR-IQ dataset. The dataset comprises 11,164 papers collected from three major machine learning conferences (ICLR 2024, ICLR 2025, and NeurIPS 2024), spanning diverse acceptance categories and research topics. }
    \label{fig:dataset_statistics}
\end{figure*}



Following the idea formalization framework introduced in the previous subsection, we now describe in detail how we extract and formalize research ideas from full academic papers. For each paper, we parsed all textual content and employed a LLM to extract structured components, including Main Target, Core Breakthrough, Innovative Methods, and Experimental Design. These components provide a standardized representation of each research idea, enabling consistent downstream evaluation and facilitating subsequent scoring procedures. A more detailed description of the prompting strategy and extraction process is provided in Appendix~\ref{app:paper_formalization}.



Next, we address potential biases in the collected ratings. Since different venues and years may exhibit systematic differences in reviewer behavior, the resulting score distributions can vary significantly across the dataset. To ensure that the scores of all papers are comparable and the overall distribution is consistent, we perform \textbf{score debiasing} using a mean-shifting procedure.


\begin{table}
\resizebox{0.48\textwidth}{!}{
  \centering
  \begin{tabular}{lccc}
    
\toprule
     & \textbf{Rating} & \textbf{Contribution} & \textbf{Soundness} \\
    \midrule
    ICLR 2024     & 2.740 & 2.689 & 2.472          \\
    ICLR 2025    & 2.821 & 2.687 & 2.498          \\
    NeurIPS 2024     & 2.918 & 2.914 & 2.721           \\
    all     & 2.825 & 2.758 & 2.559           \\
    
\bottomrule
  \end{tabular}
 }
  \caption{Average scores of papers from different venues in terms of rating, contribution, and soundness. The values highlight systematic differences across conferences and years, motivating the need for score debiasing. }
  \label{tab:debia}

\end{table}



Specifically, let $s_{i}^{(v)}$ denote the original score (rating, contribution, or soundness) of paper $i$ from venue $v$, with venue mean $\mu_v$ and overall mean $\mu_{\text{all}}$. The debiased score is computed as

\begin{equation}
\label{eq: score_debias}
\hat{s}_{i}^{(v)} = s_{i}^{(v)} - \mu_v + \mu_{\text{all}}.
\end{equation}
This procedure aligns the score distributions across different venues and years, ensuring that subsequent evaluations reflect the intrinsic quality of each idea rather than systematic biases in reviewer ratings. Additionally, the dataset was further processed through embedding computation to facilitate downstream evaluation tasks.


\subsection{Pairwise Comparison}
\label{sec:pairwise}

When a new research idea is submitted for evaluation, we first transform it into a formalized representation using the same procedure described in the previous subsection. This ensures that the target idea and reference papers are represented in a unified format.

Based on this representation, we retrieve semantically related papers from the database using a parallel retrieval strategy that combines keyword matching and embedding-based similarity. The target idea is then compared pairwise with each retrieved paper using a large language model, which assesses relative quality along three dimensions: \textit{rating}, \textit{contribution}, and \textit{soundness}.

We update the target idea's scores using an adapted Elo rating algorithm. In standard Elo, the expected probability that idea $A$ wins over idea $B$ is:
\begin{equation}
    E_A = \frac{1}{1 + 10^{(s_B - s_A) / d}},
\end{equation}
where $s_A$ and $s_B$ denote the current scores of ideas $A$ and $B$, and $d$ is a scaling parameter. Given the observed outcome $S_A \in \{0, 0.5, 1\}$, the score is updated as:
\begin{equation}
    s_A^{\text{new}} = \mathcal{C}\left(s_A + K \cdot (S_A - E_A)\right),
\end{equation}
where $K$ is an adaptive update factor and $\mathcal{C}(\cdot)$ is a soft clamping function that constrains scores to $[0, 5]$.

Through multiple rounds of pairwise comparisons, the target idea's scores gradually converge. The evaluation terminates when score changes fall below a predefined threshold, yielding the final assessment. A detailed mathematical analysis of the algorithm, including convergence properties and parameter selection, is provided in Appendix~\ref{appendix:elo}.

\subsection{Novelty Assessment}
Through the above procedures, we obtain objective evaluations of research ideas in terms of \textit{rating}, \textit{contribution}, and \textit{soundness}. However, these dimensions do not explicitly capture the \textit{novelty} of an idea. Unlike other evaluation dimensions that can be assessed through comparative analysis, novelty requires determining whether an idea introduces genuinely new insights compared to existing literature.

To address this challenge, we design a novelty assessment module that combines LLM-based initial estimation with similarity-based quantitative analysis. The evaluation proceeds in three stages: initialization, similarity measurement, and continuous fusion.

\paragraph{Initialization.} 
We first obtain an initial novelty estimate $s_{\text{novelty}}^{(0)}$ from the LLM evaluator. This provides a baseline assessment based on the model's understanding of the idea's originality and potential to introduce new insights. The LLM is prompted to rate novelty on a 0-5 scale, considering whether the approach incorporates eye-catching aspects or methods not commonly seen in the field.

\paragraph{Similarity-Based Quantification.} 
To objectively measure novelty against the current research landscape, we retrieve semantically related papers using the Semantic Scholar API. Based on the formalized representation of the target idea, we search for the most relevant publications and compute their cosine similarities $\{s_1, s_2, \ldots, s_N\}$ with the target idea using pre-trained embedding models. We then construct a weighted similarity metric:
\begin{equation}
    s_{\text{weighted}} = \alpha \cdot \max(\{s_i\}) + (1-\alpha) \cdot \frac{1}{N}\sum_{i=1}^{N} s_i,
\end{equation}
where $\alpha=0.6$ emphasizes the maximum similarity, as high similarity to even a single existing work indicates limited novelty. This weighted metric is then mapped to a novelty score through an inverse sigmoid function:
\begin{equation}
    s_{\text{sim}} = 5 \cdot \left(1 - \frac{1}{1 + e^{-k(s_{\text{weighted}} - \mu)}}\right),
\end{equation}
where $k=12$ controls the steepness of the transition, and $\mu=0.72$ defines the inflection point such that $s_{\text{weighted}}=0.72$ corresponds to moderate novelty ($s_{\text{sim}}=2.5$). This continuous mapping ensures that high similarity to existing work leads to low novelty scores, while low similarity indicates high novelty.

\paragraph{Continuous Fusion.} 
The final novelty score integrates both the LLM's subjective assessment and the objective similarity-based measurement:
\begin{equation}
    s_{\text{novelty}}^{\text{final}} = \beta \cdot s_{\text{sim}} + (1-\beta) \cdot s_{\text{novelty}}^{(0)},
\end{equation}
where $\beta=0.7$ assigns higher weight to the similarity-based calculation, reflecting its objectivity, while retaining the LLM's judgment to capture aspects not fully represented by semantic similarity alone.

Through this approach, our novelty assessment combines the semantic understanding of language models with quantitative similarity analysis, producing continuous scores that effectively distinguish ideas across the full novelty spectrum.

==> text/4.experiments.tex <==
\section{Experiments}
\subsection{Model Training}

\begin{table}
\small
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.0}
  \centering
  \begin{tabular}{lccc}
    \toprule
    \textbf{Model} & \textbf{Rating} & \textbf{Contrib.} & \textbf{Sound.} \\
    \midrule
    Qwen2.5-7B     & 0.514 & 0.496 & 0.488          \\
    Qwen2.5-14B    & 0.506 & 0.598 &0.541\\
    GPT-4o & 0.549 & 0.615 & 0.747\\
    GPT-4.1     & 0.539 & 0.545 & 0.649         \\
    GPT-5     & \textbf{0.820} & 0.695 & \textbf{0.826}           \\
    GPT-5.2 & 0.801 & 0.707 & 0.803 \\
    Gemini-2.5-pro & 0.706 & 0.607 & 0.750 \\
    Gemini-3-pro & 0.806 & 0.\textbf{713} &  0.814\\
    \midrule
    Qwen2.5-7B(trained)     & 0.714 & 0.710 & 0.712           \\
    Qwen2.5-14B(trained)     & 0.755 & 0.701 & 0.751           \\
    \bottomrule
  \end{tabular}
  \caption{Accuracy of LLM-based pairwise judgments on \textit{rating}, \textit{contribution}, and \textit{soundness}, evaluated against debiased OpenReview ground-truth labels.}
  \label{tab:pairwise_eval}
\end{table}


We also fine-tune models of smaller sizes to investigate whether the scientific "taste" of an area can be learned through knowledge distillation. Following Section~\ref{sec:pairwise_evaluation}, we sample \num{15000} thematically similar pairs while ensuring none of the selected papers appear in the test data. To help small models better understand the underlying domain knowledge, we adopt an additional chain-of-thought~\cite{cot} generated by larger models based on ground-truth labels. We choose Qwen2.5-72B-Instruct~\cite{qwen25} as the teacher model, and smaller models from the same family as the student models. As for the training framework, we employ LLaMA-Factory~\cite{llamafactory}, and further details are presented in Appendix~\ref{app:training_hyperparameter}.



\subsection{Pairwise Evaluation}

\label{sec:pairwise_evaluation}



The accuracy of pairwise judgments made by the LLM serves as a key guarantee for the reliability of the entire evaluation framework. To assess this reliability, we conduct a dedicated pairwise evaluation on the three dimensions: \textit{rating}, \textit{contribution}, and \textit{soundness}. The goal of this evaluation is to verify whether the LLM can correctly determine the relative quality between two research ideas under each criterion.

For this purpose, we randomly sample a held-out test set consisting of 269 pairs of thematically similar papers from the database, ensuring that none of the selected papers appear in the training data. Thematic similarity is determined using the same hybrid retrieval strategy based on keyword matching and embedding-based similarity. Each sampled pair is presented to the LLM in its formalized representation, and the model is asked to judge which idea performs better on each of the three dimensions.

The ground-truth labels for pairwise comparison are derived from the \textbf{debiased OpenReview scores}. Specifically, for each paper pair, we compare their debiased scores on \textit{rating}, \textit{contribution}, and \textit{soundness}, and treat the resulting relative ordering as the reference outcome. The accuracy of the LLM’s pairwise judgments is then measured by comparing its predictions against these ground-truth relationships, as summarized in Table~\ref{tab:pairwise_eval}.




Overall, stronger models consistently achieve higher accuracy across all three dimensions, indicating that pairwise judgment is a non-trivial capability that benefits from increased model capacity and reasoning ability. Among the off-the-shelf models, \texttt{gpt-5} substantially outperforms other baselines, achieving accuracies above 0.80 on both \textit{rating} and \textit{soundness}, which suggests a high level of agreement with debiased human judgments.

In contrast, smaller open-source models such as Qwen2.5-7B and Qwen2.5-14B exhibit limited performance, with accuracies close to random guessing in some dimensions, particularly on \textit{rating} and \textit{soundness}. This highlights the difficulty of reliably performing fine-grained comparative evaluation without sufficient model capacity or task-specific supervision.

Notably, models trained on the PAIR-IQ dataset show substantial improvements across all dimensions. Both trained variants achieve consistently higher accuracies than their untrained counterparts, demonstrating that targeted pairwise supervision effectively enhances the model’s ability to align with human evaluation criteria. These results validate the design of the PAIR-IQ dataset and further support the use of pairwise judgment as a reliable component within the LigBench evaluation framework.

Although the pairwise judgment accuracy does not reach near-perfect levels, this outcome also reflects the intrinsic difficulty of the task, as distinguishing fine-grained differences between closely related research ideas is inherently challenging. Nevertheless, when applied within the LigBench framework, even imperfect pairwise judgments can still lead to reliable final evaluations. Starting from a strong base model, repeated score updates over a large number of pairwise comparisons allow the target scores to gradually converge toward reasonable values.

\begin{table}
\small
  \centering
  \begin{tabular}{ccc}
    \toprule
     \textbf{Rating} & \textbf{Contrib.} & \textbf{Sound.} \\
    \midrule
     0.114 & 0.196 & 0.138          \\
    \bottomrule
    
  \end{tabular}
  \caption{Mean debiased score differences for incorrectly judged paper pairs by \textbf{GPT-5} in the pairwise evaluation. The small score gaps indicate that errors have limited impact on iterative score updates.}
  \label{tab:error_analysis}
\end{table}

Further analysis of the error cases, summarized in Table~\ref{tab:error_analysis}, reveals that most incorrect judgments occur when the debiased scores of the two compared papers are very close. This observation suggests that even when the LLM makes an incorrect decision, the resulting update magnitude is limited. According to the score update mechanism described in the previous section, such small score differences lead to correspondingly small update steps, thereby preventing severe error accumulation during the iterative evaluation process.



\subsection{Human Alignment}
Although the pairwise judgment capability of the large language model has been validated using debiased OpenReview scores, it remains essential to perform human verification. This is because even debiased scores cannot guarantee a perfectly objective assessment, and expert judgment is required to ensure alignment with human evaluation standards.

To further verify human alignment, we recruited several PhD-level AI researchers to conduct pairwise comparisons on \textbf{100 randomly sampled idea pairs}. For each pair, experts selected the superior idea along the three dimensions: \textit{rating}, \textit{contribution}, and \textit{soundness}. The resulting human judgments were then compared with the LLM’s pairwise predictions. The alignment results are summarized in Table~\ref{tab:human_alignment}, indicating a strong consistency between the LLM and expert evaluations.

\begin{table}
\small
  \centering
  \begin{tabular}{ccc}
    \toprule
     \textbf{Rating} & \textbf{Contrib.} & \textbf{Sound.} \\
    \midrule
    71\% & 79\% & 73\%         \\
   
    \bottomrule
    
  \end{tabular}
  \caption{Agreement between LLM-based pairwise judgments and human expert evaluations across three assessment dimensions. Values denote the proportion of pairwise decisions consistent with PhD-level expert judgments.}
  \label{tab:human_alignment}
\end{table}

As shown in Table~\ref{tab:human_alignment}, the LLM exhibits substantial agreement with human experts across all three dimensions. In particular, the highest alignment is observed for \textit{contribution}, indicating that the model is effective at assessing the relative significance of research ideas within a domain. The consistently strong agreement on \textit{rating} and \textit{soundness} further suggests that the LLM’s pairwise judgments capture key aspects of overall quality and methodological rigor. These results provide additional evidence that LigBench produces evaluations that are well aligned with expert human preferences, complementing the automated assessments based on debiased review scores.

\subsection{Paper Evaluation}
We conducted an evaluation on papers from \textbf{NeurIPS 2025} to demonstrate the effectiveness of our framework. The evaluation applied the full LigBench procedure. The results of this evaluation are summarized in Table~\ref{tab:nips2025_evaluation}, highlighting the performance of the framework across the different assessment dimensions.

% 明瑄找一点nips2025的文章测一下，仅按照accept/reject来区分

\begin{table}
\small
  \centering
  \begin{tabular}{lcc}
   \toprule
     & \textbf{Accept} & \textbf{Reject} \\
    \midrule
    Rating & 2.547 & 2.043           \\
    Contribution & 2.432 & 2.030   \\
    Soundness & 1.853 & 1.542   \\
    Novelty & 2.627 & 2.234   \\
    \bottomrule
    
  \end{tabular}
  \caption{Evaluation of 50 NeurIPS 2025 papers using LigBench. Each score represents the average assessment of the papers on \textit{rating}, \textit{contribution}, \textit{soundness}, and \textit{novelty}.}
  \label{tab:nips2025_evaluation}
\end{table}

As shown in Table~\ref{tab:nips2025_evaluation}, papers that were accepted at NeurIPS 2025 consistently receive higher scores across all four evaluation dimensions compared to rejected papers. The largest differences are observed in \textit{novelty} and \textit{rating}, suggesting that both originality and overall perceived quality are strong determinants of acceptance. Differences in \textit{contribution} and \textit{soundness} are also notable, indicating that methodological rigor and domain impact are effectively captured by LigBench.

These results demonstrate that LigBench can meaningfully distinguish higher-quality research ideas from lower-quality ones, even when applied to a relatively small test set of 50 papers. This alignment with actual acceptance outcomes provides preliminary validation of the framework’s effectiveness in reflecting human and peer-review judgments.


\subsection{Benchmark and Model Evaluation}

To comprehensively assess the quality of LLM-generated research ideas, we evaluate both standalone LLMs and idea-generation frameworks using LigBench. Each system is prompted to freely generate 10 ideas across 11 research topics, including Reinforcement Learning, Image Generation, AI Safety, Agent, Computer Vision, Audio and Speech, Embodied Intelligence, Multimodal, AI for Science, Large Language Models, and Training. The final score for each model is computed as the average across all generated ideas.

We compare two representative idea-generation frameworks, CoI and SciPIP, against direct LLM baselines. Both frameworks employ GPT-5 as their underlying language model, enabling a controlled comparison that isolates the contribution of framework design from model capability. The evaluation results are summarized in Table~\ref{tab:benchmark}.

\begin{table}[t]
\centering
\small
\begin{tabular}{lcccc}
\toprule
\textbf{Model} & \textbf{Rating} & \textbf{Contrib.} & \textbf{Sound.} & \textbf{Novelty} \\
\midrule
CoI & 3.468 & 2.996 & 2.487 & 2.474 \\
SciPIP & 2.621 & 1.900 & \textbf{3.243} & 2.267 \\
\midrule
GPT-5.2 & \textbf{3.974} & \textbf{3.392} & 3.022 & \textbf{2.583} \\
GPT-5 & 3.686 & 3.210 & 2.866 & 2.528 \\
GPT-4.1 & 1.000 & 0.760 & 1.877 & 2.194 \\
GPT-4o & 0.672 & 0.514 & 1.264 & 1.877 \\

\bottomrule
\end{tabular}
\caption{Evaluation of idea-generation frameworks and standalone LLMs using LigBench. Scores are averaged across 110 generated ideas per model. CoI\cite{coi} and SciPIP\cite{scipip} both use GPT-5 as the backbone model.}
\label{tab:benchmark}
\end{table}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\linewidth]{figure/radar.png}
    \caption{Radar chart visualization of Table~\ref{tab:benchmark}. GPT-5.2 achieves the highest overall performance, while CoI demonstrates competitive results despite using GPT-5 as its backbone.}
    \label{fig:radar}
\end{figure}

Several observations emerge from these results. First, among standalone LLMs, we observe a clear performance hierarchy aligned with model capability: GPT-5.2 and GPT-5 substantially outperform GPT-4.1 and GPT-4o across all dimensions, with GPT-4o scoring below 1.0 on rating and contribution, indicating that earlier-generation models struggle to meet basic quality thresholds.

Second, an unexpected finding is that idea-generation frameworks do not consistently outperform direct prompting when applied to strong backbone models. Despite using GPT-5 as their underlying model, both CoI and SciPIP achieve lower scores than standalone GPT-5 on most dimensions. This suggests that these frameworks may have been optimized for enhancing weaker models, and their structured pipelines introduce constraints that limit the performance ceiling of already-capable models. Notably, SciPIP attains a higher score on the Soundness dimension than its underlying model GPT-5, and achieves the highest soundness score among all evaluated systems and models, indicating that its design contributes positively to methodological rigor despite the overall performance trade-offs.

Finally, although the novelty scores of the various models and frameworks exhibit an ordering that is broadly consistent with our expectations, the absolute differences between their scores are relatively small. This observation also suggests, from another perspective, that for current LLMs, generating a truly novel idea remains a non-trivial challenge.

% To fully explore the creative potential of each evaluated framework or agent, our benchmark prompts them to freely generate 10 ideas for each of 11 specified topics: \textit{Reinforcement Learning}, \textit{Image Generation}, \textit{AI Safety}, \textit{Agent}, \textit{Computer Vision}, \textit{Audio and Speech}, \textit{Embodied Intelligence}, \textit{Multimodal}, \textit{AI for Science}, \textit{Large Language Models}, and \textit{Training}. The generated ideas are then assessed using the LigBench framework, and the final evaluation score for each topic is computed as the mean over the 10 generated ideas.

% We evaluated a range of state-of-the-art idea generation frameworks using \textbf{LigBench} to assess the quality of the ideas they produced. In addition, we also evaluated ideas generated directly by LLMs without any additional framework to provide a baseline comparison. The evaluation covered all relevant dimensions, including \textit{rating}, \textit{contribution}, \textit{soundness}, and \textit{novelty}. The results of this evaluation are summarized in Table~\ref{tab:model_evaluation}, highlighting the relative performance of different models and the effectiveness of our framework in producing high-quality research ideas.

% 参考https://arxiv.org/pdf/2512.16969里面测评的工作

==> text/5.conclusion.tex <==
\section{Conclusion}

We introduced \textbf{LigBench}, a unified and human-aligned benchmark for evaluating research ideas generated by large language models and agentic frameworks. By decomposing idea quality into four dimensions—\textit{rating}, \textit{contribution}, \textit{soundness}, and \textit{novelty}, LigBench enables consistent and fine-grained assessment across diverse idea sources.

To support reliable evaluation, we constructed the \textbf{PAIR-IQ} dataset with standardized and debiased scores, enabling effective pairwise judgment and robust score updating. Experimental results show that LigBench produces stable evaluations aligned with expert preferences, even when individual pairwise judgments are imperfect.

We believe LigBench provides a practical foundation for benchmarking future idea-generation systems and advances the automated evaluation of scientific creativity.


\section{Limitations}

Despite its effectiveness, LigBench has several limitations. The framework relies on the pairwise judgment capability of large language models to compare research ideas across multiple dimensions. While our experiments show strong agreement with debiased OpenReview scores and human expert judgments, pairwise comparison remains inherently challenging, particularly when differences between ideas are subtle or when ideas are closely related. In addition, LigBench depends on a static database of existing papers for reference-based evaluation and score propagation. Although the use of a large and diverse corpus improves robustness, ideas from newly emerging research areas or those that substantially deviate from existing literature may be less accurately assessed due to limited relevant references.
